Blockchain Bribing Attacks and the Efficacy of Counterincentives

We analyze bribing attacks in Proof-of-Stake distributed ledgers from a game theoretic perspective. In bribing attacks, an adversary offers participants a reward in exchange for instructing them how to behave, with the goal of attacking the protocol's properties. Specifically, our work focuses on adversaries that target blockchain safety. We consider two types of bribing, depending on how the bribes are awarded: i) guided bribing, where the bribe is given as long as the bribed party behaves as instructed; ii) effective bribing, where bribes are conditional on the attack's success, w.r.t. well-defined metrics. We analyze each type of attack in a game theoretic setting and identify relevant equilibria. In guided bribing, we show that the protocol is not an equilibrium and then describe good equilibria, where the attack is unsuccessful, and a negative one, where all parties are bribed such that the attack succeeds. In effective bribing, we show that both the protocol and the "all bribed" setting are equilibria. Using the identified equilibria, we then compute bounds on the Prices of Stability and Anarchy. Our results indicate that additional mitigations are needed for guided bribing, so our analysis concludes with incentive-based mitigation techniques, namely slashing and dilution. Here, we present two positive results, that both render the protocol an equilibrium and achieve maximal welfare for all parties, and a negative result, wherein an attack becomes more plausible if it severely affects the ledger's token's market price.

==> sections/bribing_coor.tex <==
\subsection{Coordinated bribing attacks}\label{subsec:bribing_coor}
We study the scenario where the briber  issues the parties' external rewards in a way that  the double-signing becomes effective (i.e., lead to the drop of the exchange rate). This implies some level of coordination among parties. Formally, for some fixed slot $\slot$ and time span $\Delta\geq0$, the external rewards are defined as
 \begin{equation}\label{eq:external_coor}
\utilityBoost_{\party,\profile}(\trace)=\left\{\begin{array}{ll}\beta_\party,& \mbox{if in $\trace$, }\party\mbox{ double-signs in }[\slot,\slot+\Delta]\\
0,&\mbox{otherwise}\end{array}\right.\;.
\end{equation}

In our study, we introduce the notion of an $\infractionPredicate_\mathsf{ds}$-agnostic strategy profile. 

\begin{definition}\label{def:ds_agnostic}
A strategy profile $\profile$ is \emph{$\infractionPredicate_\mathsf{ds}$-agnostic}, if for every $i,j\in[n]:i\neq j$, the strategy of $\party_i$ does not depend on the double-signing activity of $\party_j$ during the execution.
\end{definition}
Intuitively, the strategy of $\party_i$ in the $\infractionPredicate_\mathsf{ds}$-agnostic strategy profile $\profile$ does not contain clauses such as ``I will double-sign if $\party_j$ does not double-sign'', ``I will not double-sign, if everyone else has already double-signed'', etc.
%In the following theorem, we prove that in the coordinated setting, the strategy $\strategy_\mathsf{ds}^{\slot,\Delta}$ strictly dominates every $\infractionPredicate_\mathsf{ds}$-agnostic strategy profile, if the party's bribe is sufficiently large.

\begin{theorem}\label{thm:coor}
Let $\proto$ be a protocol with block-proportional rewards (cf. Subsection~\ref{subsec:preliminaries_proportion}) with $\reward$ rewards per block. Let $\profile_\proto$ denote the all-honest strategy profile. Assume that for any strategy profile $\sigma$, the exchange rate $\exchangeRate_\profile$ is defined as in Eq.~\eqref{eq:exchange} and the external rewards $\utilityBoost_{\party,\profile}$ due to coordinated bribing \wrt a slot $\slot$ and timespan $\Delta$ are defined as in Eq.~\eqref{eq:external_coor}. Let $\adversary$ be a synchronous router. Then, the following hold:
%
\begin{enumerate}
%\item\label{thm:nocoor_nash} For every slot $\slot$, the strategy profile  $\profile_\mathsf{ds}^{\slot,\Delta}$ is a Nash equilibrium \wrt Reward under $\adversary$.$\forall\party\in\partySet:\big(\power_\party>\frac{1}{2}\Rightarrow\beta_\party\geq E[\reward_{\party, \profile_\proto}]\cdot x\big)$ if and only if 
\item\label{thm:coor_nash1} If for every party $\party\in\partySet$, it holds that $\power_\party<\frac{1}{2}$, then, there is an  $\epsilon$ negligible in $\secparam$ such that the strategy profile  $\profile_\mathsf{ds}^{\slot,\Delta}$ is an $\epsilon$-Nash equilibrium \wrt Reward under $\adversary$.\TZ{Completed}
%
\item\label{thm:coor_nash2}  Assume that there is a (unique) party $\party\in\partySet$ such that $\power_\party>\frac{1}{2}$. Let $\theta>0$ be a real value such that the probability $\Pr\big[\msgNumber_{\party, \profile_\proto}>(1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\big]$ is negligible in $\secparam$, where $\msgNumber_{\party, \profile_\proto}$ is the number of blocks created by $\party$ in $\profile_\proto$. If $\beta_\party\geq (1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\cdot\reward\cdot x$, then there is an  $\epsilon$ negligible in $\secparam$ such that the strategy profile  $\profile_\mathsf{ds}^{\slot,\Delta}$ is an $\epsilon$-Nash equilibrium \wrt Reward under $\adversary$.\TZ{Completed.}
%
\item\label{thm:coor_compliance} If there is a party $\party\in\partySet$ such that $\power_\party\leq\frac{1}{2}$ and $\beta_\party\geq \big(E[\msgNumber_{\party, \profile_\proto}^\Delta]+1\big)\cdot\reward\cdot x$, where $\msgNumber_{\party, \profile_\proto}^\Delta$ is the number of blocks created by $\party$ during a timespan $\Delta$ in $\profile_\proto$, then for every $0\leq\epsilon\leq\beta_\party-( E[\msgNumber_{\party, \profile_\proto}^\Delta]+1)\cdot\reward\cdot x$, $\proto$ is not $(\epsilon,\infractionPredicate_\mathsf{ds})$-compliant \wrt Reward under $\adversary$.\TZ{Completed}
%
\item\label{thm:coor_reachable} Let $\theta>0$ be a real value such that the probability $\Pr\big[\msgNumber_{\party, \profile_\proto}>(1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\big]$ is negligible in $\secparam$, where $\msgNumber_{\party, \profile_\proto}$ is the number of blocks created by $\party$ in $\profile_\proto$. If $\beta_\party\geq(1+\theta)\cdot\big( E[\msgNumber_{\party, \profile_\proto}]+1\big)\cdot \reward\cdot x$ for every party $\party\in\partySet$,  then for every $0\leq\epsilon\leq\underset{j\in[n]}{\mathsf{min}}\big\{\beta_{\party_j}-(1+\theta)\cdot\big(E[\msgNumber_{\party_j, \profile_\proto}]\cdot\reward+1\big)\cdot x\big\}$,  $\profile_\mathsf{ds}^{\slot,\Delta}$ is $\epsilon$-reachable from $\profile_\proto$ \wrt Reward under $\adversary$.\TZ{Not sure if this holds}
\end{enumerate}
\end{theorem}

\begin{proof}
\ref{thm:coor_nash1}. The proof is similar to \ref{thm:nocoor_nash1} of Theorem~\ref{thm:nocoor}. Here, the slot $\slot$ is fixed according to Eq.~\eqref{eq:external_coor}.\\

\ref{thm:coor_nash2}. The proof is similar to \ref{thm:nocoor_nash2} of Theorem~\ref{thm:nocoor}. Here, the slot $\slot$ is fixed according to Eq.~\eqref{eq:external_coor}.\\

\ref{thm:coor_compliance}. The proof is similar to \ref{thm:nocoor_compliance} of Theorem~\ref{thm:nocoor}. \\

\ref{thm:coor_reachable}. We define the strategy profiles $\profile_j^\slot$, $j\in\{0,\ldots,n\}$  as in the proof of~\ref{thm:nocoor_compliance}. in Theorem~\ref{thm:nocoor}. 

\end{proof}







\ignore{
\begin{proof}
We define the strategy profiles $\profile_j^\slot$, $j\in\{0,\ldots,n\}$  as in the proof of~\ref{thm:nocoor_compliance}. in Theorem~\ref{thm:nocoor}. Similarly, we can show that for every $j\in[n]$: (a) $\profile_j^\slot$ is unilateral deviation of $\party_j$ from $\profile_{j-1}^\slot$ and (b) $\utility_\party(\profile_j^\slot)> \utility_\party(\profile_{j-1}^\slot)$. By the definition of reachability, it suffices to show that for every $j\in[n]$, $\profile_j^\slot$ sets a best response for $\party_j$.

Let $\profile^*$ be a unilateral deviation of $\party_j$ from $\profile_{j-1}^\slot$. By definition of $\strategy_\mathsf{ds}^{\slot,\Delta}$, $\profile_{j-1}^\slot$ is $\infractionPredicate_\mathsf{ds}$-agnostic, thus all the other parties' strategies in  $\profile^*$ (which are the same as in  $\profile_{j-1}^\slot$) do not depend on the double-signing activity of $\party_j$. Given the latter, we study the following cases:

\emph{Case 1}:  By unilaterally deviating from  $\profile_{j-1}^\slot$ to  $\profile_j^\slot$, the party $\party_j$'s double-signing  in slot $\slot$ does not affect the exchange rate. Then, the same holds for $\profile^*$. Let $D_\slot$ be the event that $\party_j$ double-signs in slot $\slot$ when following $\profile^*$. If the rate in $\profile_{j-1}^\slot$ and  $\profile_j^\slot$ is $c\in\{0,x\}$, we have that,
\begin{equation*}
\begin{split}
\utility_{\party_j}(\profile^*)&=\sum_z z\cdot\big(\Pr[D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot\exchangeRate_{\profile^*}+\utilityBoost_{\party_j, \profile^*}=z\mid D_\slot]+\\
&\quad+\Pr[\neg D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot\exchangeRate_{\profile^*}+\utilityBoost_{\party_j, \profile^*}=z\mid \neg D_\slot]\big)=\\
%
&\mbox{\TZ{Here, the proof breaks...:(}}\\
%
&=\sum_z z\cdot\big(\Pr[D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot c+\beta_{\party_j}=z]+\\
&\quad+\Pr[\neg D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot c=z]\big)=\\
%
&=\Pr[D_\slot]\cdot E[\reward_{\party_j, \profile^*}\cdot c+\beta_{\party_j}]+\Pr[\neg D_\slot]\cdot E[\reward_{\party_j, \profile^*}\cdot c]=\\
%
&= E[\reward_{\party_j, \profile^*}]\cdot c+\Pr[D_\slot]\cdot\beta_{\party_j}\leq E[\reward_{\party_j, \profile_\proto}]\cdot c+\beta_{\party_j}=\\
%
&=E[\reward_{\party_j, \profile_j^\slot}]\cdot c+\beta_{\party_j}=\utility_{\party_j}(\profile_j^\slot).
\end{split}
\end{equation*} 
%
\indent\emph{Case 2}:  By unilaterally deviating from  $\profile_{j-1}^\slot$ to  $\profile_j^\slot$, the party $\party_j$'s double-signing affects the exchange rate. In this case, by the definition of $\profile_1^\slot,\ldots,\profile_n^\slot$, it holds that 
%
\[\sum_{w=1}^{j-1}\power_{\party_w}\leq\frac{1}{2}\wedge\sum_{w=1}^{j}\power_{\party_w}>\frac{1}{2}.\]
%
Thus, if $D_\slot$ happens, then the exchange rate is $0$ and the external rewards of $\party_j$ are $\beta_{\party_j}$. If $D_\slot$ does not happen then the exchange rate is $x$ and, because we are in the coordinated setting, the external rewards of $\party_j$ are $0$. We have that
\begin{equation*}
\begin{split}
\utility_{\party_j}(\profile^*)&=\sum_z z\cdot\big(\Pr[D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot\exchangeRate_{\profile^*}+\utilityBoost_{\party_j, \profile^*}=z\mid D_\slot]+\\
&\quad+\Pr[\neg D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot\exchangeRate_{\profile^*}+\utilityBoost_{\party_j, \profile^*}=z\mid \neg D_\slot]\big)=\\
%
&=\sum_z z\cdot\big(\Pr[D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot 0+\beta_{\party_j}=z]+\\
&\quad+\Pr[\neg D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot x+0=z]\big)=\\
%
&=\Pr[D_\slot]\cdot \beta_{\party_j}+\Pr[\neg D_\slot]\cdot E[\reward_{\party_j, \profile^*}\cdot x]\leq\\
%
&\leq \mathsf{max}\{\beta_{\party_j}, E[\reward_{\party_j, \profile_\proto}]\cdot c\}=\beta_{\party_j}=\utility_{\party_j}(\profile_j^\slot).
\end{split}
\end{equation*} 
\end{proof}
}

==> sections/bribing_nocoor.tex <==
\subsection{Non-coordinated bribing attacks}\label{subsec:bribing_nocoor}
In the non-coordinated setting, the briber tempts the parties to double-sign by offering them an amount of external rewards if they do at any preferred moment. This is formalized as follows: %\TZ{We do not need to define the external rewards \wrt some specific slot $\slot$. Coordination of the parties regarding when they double sign is specified by the strategy profile.}

\begin{equation}\label{eq:external}
\utilityBoost_{\party,\profile}(\trace)=\left\{\begin{array}{ll}\beta_\party,& \mbox{if in $\trace$, there is a slot }\slot: \party\mbox{ double-signs in }\slot\\
0,&\mbox{otherwise}\end{array}\right.\;,
\end{equation}
%
where $\beta_\party$ is some positive constant.  

In the following theorem, we prove that under non-coordinated bribing, a synchronous network, block-proportional rewards with $\reward$ rewards per block, and the Reward utility function:
\begin{enumerate}
\item  $\profile_\mathsf{ds}^{\slot,\Delta}$ is a $\negl(\secparam)$-Nash equilibrium if every party holds less than half of the majority of the participation power.

\item  $\profile_\mathsf{ds}^{\slot,\Delta}$ is a $\negl(\secparam)$-Nash equilibrium if there is  a party that holds the majority of participation power, but her bribe is sufficiently large (it substantially exceeds the expected number of blocks that the party creates, multiplied by $\reward\cdot x$).
%
\item The protocol $\proto$ is not  $\infractionPredicate_\mathsf{ds}$-compliant, if there is a party $\party$ that does not hold the majority of the participation power, but her bribe exceeds the expected system's expected number of blocks that $\party$ creates during a timespan $\Delta$., multiplied by $\reward\cdot x$. For instance, in Bitcoin this lower bound for the bribe is $\delta\cdot\power_\party\cdot q\cdot(\Delta+1)\cdot\reward\cdot x$, where $\delta$ is the success probability of a hashing query and $\power_\party\cdot q$ is available queries of $\party$ per slot. In PoS, this lower bound is $\power_\party\cdot(\Delta+1)\cdot\reward\cdot x$.
%
\item  $\profile_\mathsf{ds}^{\slot,\Delta}$ is weakly reachable from the all honest strategy profile under the stronger condition that the bribe for all parties is sufficiently large (it  exceeds the expected number of blocks that the party creates, multiplied by $\reward\cdot x$).\TZ{By ``weakly'' I mean that the players do not move only to best responses. If this result makes sense, we can add the definition of ``weak'' reachability.}
\end{enumerate}

\begin{theorem}\label{thm:nocoor}
Let $\proto$ be a protocol with block-proportional rewards (cf. Subsection~\ref{subsec:preliminaries_proportion}) with $\reward$ rewards per block. Let $\profile_\proto$ denote the all-honest strategy profile. Assume that for any strategy profile $\sigma$, the exchange rate $\exchangeRate_\profile$ is defined as in Eq.~\eqref{eq:exchange} and the external rewards $\utilityBoost_{\party,\profile}$ due to non-coordinated bribing \wrt timespan $\Delta$ are defined as in Eq.~\eqref{eq:external}. Let $\adversary$ be a synchronous router. Then, the following hold:
%
\begin{enumerate}
%\item\label{thm:nocoor_nash} For every slot $\slot$, the strategy profile  $\profile_\mathsf{ds}^{\slot,\Delta}$ is a Nash equilibrium \wrt Reward under $\adversary$.$\forall\party\in\partySet:\big(\power_\party>\frac{1}{2}\Rightarrow\beta_\party\geq E[\reward_{\party, \profile_\proto}]\cdot x\big)$ if and only if 
\item\label{thm:nocoor_nash1} If for every party $\party\in\partySet$, it holds that $\power_\party<\frac{1}{2}$, then for every slot $\slot$, there is an  $\epsilon$ negligible in $\secparam$ such that the strategy profile  $\profile_\mathsf{ds}^{\slot,\Delta}$ is an $\epsilon$-Nash equilibrium \wrt Reward under $\adversary$.\TZ{Completed}
%
\item\label{thm:nocoor_nash2}  Assume that there is a (unique) party $\party\in\partySet$ such that $\power_\party>\frac{1}{2}$. Let $\theta>0$ be a real value such that the probability $\Pr\big[\msgNumber_{\party, \profile_\proto}>(1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\big]$ is negligible in $\secparam$, where $\msgNumber_{\party, \profile_\proto}$ is the number of blocks created by $\party$ in $\profile_\proto$. If $\beta_\party\geq (1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\cdot\reward\cdot x$, then for every slot $\slot$, there is an  $\epsilon$ negligible in $\secparam$ such that the strategy profile  $\profile_\mathsf{ds}^{\slot,\Delta}$ is an $\epsilon$-Nash equilibrium \wrt Reward under $\adversary$.\TZ{Completed.}
%
\item\label{thm:nocoor_compliance} If there is a party $\party\in\partySet$ such that $\power_\party\leq\frac{1}{2}$ and $\beta_\party\geq \big(E[\msgNumber_{\party, \profile_\proto}^\Delta]+1\big)\cdot\reward\cdot x$, where $\msgNumber_{\party, \profile_\proto}^\Delta$ is the number of blocks created by $\party$ during a timespan $\Delta$ in $\profile_\proto$, then for every $0\leq\epsilon\leq\beta_\party-( E[\msgNumber_{\party, \profile_\proto}^\Delta]+1)\cdot\reward\cdot x$, $\proto$ is not $(\epsilon,\infractionPredicate_\mathsf{ds})$-compliant \wrt Reward under $\adversary$.\TZ{Completed}
%
\item\label{thm:nocoor_reachable} If $\beta_\party\geq\big( E[\msgNumber_{\party, \profile_\proto}]+1\big)\cdot \reward\cdot x$ for every party $\party\in\partySet$, where $\msgNumber_{\party, \profile_\proto}$ is the number of blocks created by $\party$ in $\profile_\proto$, then for every $0\leq\epsilon\leq\underset{j\in[n]}{\mathsf{min}}\big\{\beta_{\party_j}-\big(E[\msgNumber_{\party_j, \profile_\proto}]\cdot\reward+1\big)\cdot x\big\}$ and every slot $\slot$,  $\profile_\mathsf{ds}^{\slot,\Delta}$ is weakly $\epsilon$-reachable from $\profile_\proto$ \wrt Reward under $\adversary$.\TZ{Completed}
\end{enumerate}
\end{theorem}

\begin{proof}
\ref{thm:nocoor_nash1}. Assume that the parties follow $\profile_\mathsf{ds}^{\slot,\Delta}=\langle\strategy_\mathsf{ds}^{\slot,\Delta},\ldots,\strategy_\mathsf{ds}^{\slot,\Delta}\rangle$. Let $F_\party$ be the event that $\party$ fails to double-sign in $[\slot,\slot+\Delta]$, so $\Pr[F_\party]=q_\party^{\slot,\Delta}=\negl(\secparam)$. It follows that the probability of the event $\neg\bigvee_{\party\in\partySet}F_\party$ that all the parties are able to double-sign in $[\slot,\slot+\Delta]$ is
\[\Pr\Big[\neg\bigvee_{\party\in\partySet}F_\party\Big]=1-\Pr\Big[\bigvee_{\party\in\partySet}F_\party\Big]\geq 1-\sum_{\party\in\partySet}\Pr[F_\party]=1-n\cdot\negl(\secparam)=1-\negl(\secparam).\]
%
 When $\neg\bigvee_{\party\in\partySet}F_\party$ happens, all parties double-sign at some point in $[\slot,\slot+\Delta]$, so the exchange rate is $0$ and the parties take their external rewards. Thus, by Eq.~\eqref{eq:exchange} and~\eqref{eq:external}, the utility of some party $\party$ is 
\begin{equation}\label{eq:utility_ds_all}
\begin{split}
\utility_\party(\profile_\mathsf{ds}^{\slot,\Delta})&=E[\reward_{\party, \profile_\mathsf{ds}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_\mathsf{ds}^{\slot,\Delta}}]+E[\utilityBoost_{\party, \profile_\mathsf{ds}^{\slot,\Delta}}]=\\
%
&=\sum_z z\cdot\Pr[\reward_{\party, \profile_\mathsf{ds}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_\mathsf{ds}^{\slot,\Delta}}+\utilityBoost_{\party, \profile_\mathsf{ds}^{\slot,\Delta}}=z]\geq\\
%
&\geq\Pr\Big[\neg\bigvee_{\party\in\partySet}F_\party\Big]\cdot\sum_z z\cdot\Pr\Big[\reward_{\party, \profile_\mathsf{ds}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_\mathsf{ds}^{\slot,\Delta}}+\utilityBoost_{\party, \profile_\mathsf{ds}^{\slot,\Delta}}=z\Big|\neg\bigvee_{\party\in\partySet}F_\party\Big]=\\
%
&=\Pr\Big[\neg\bigvee_{\party\in\partySet}F_\party\Big]\cdot\sum_z z\cdot\Pr[\reward_{\party, \profile_\mathsf{ds}^{\slot,\Delta}}\cdot 0+\beta_\party=z]=\\
%
&=\big(1-\negl(\secparam)\big)\cdot\beta_\party=\beta_\party-\negl(\secparam).
\end{split}
\end{equation}
Assume now that some party $\party^*$ unilaterally deviates from $\profile_\mathsf{ds}^{\slot,\Delta}$ to some strategy profile $\profile$. 

By assumption, $\power_{\party^*}<\frac{1}{2}$. Observe that  all other parties, which sum of participation powers is greater than $\frac{1}{2}$, double-sign in $[\slot,\slot+\Delta]$ when following $\profile$, whenever they are able to. Thus,  when $\neg\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party$ happens, the exchange rate is $0$ no matter what the strategy of $\party^*$ is. As before, we have that $\Pr\Big[\neg\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party\Big]=1-\negl(\secparam)$. Given the fact that, under block-proportional rewards, the maximum system's rewards a party can take is polynomially bounded by $\rounds\cdot\reward$, where $\rounds$ is the number of rounds in the execution, we get that,
\begin{equation}\label{eq:utility_ds_all_deviate}
\begin{split}
\utility_{\party^*}(\profile)&=\sum_z z\cdot\Pr[\reward_{\party^*, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party^*}=z]=\\
%
&=\sum_z z\cdot\Pr\Big[\reward_{\party^*, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party^*}=z\wedge\Big(\neg\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party\Big)\Big]+\\
&\quad+\sum_z z\cdot\Pr\Big[\reward_{\party^*, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party^*}=z\wedge\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party\Big]\leq\\
%
&\leq\Big[\neg\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party\Big]\cdot\sum_z z\cdot\Pr\Big[\reward_{\party^*, \profile}\cdot 0+\utilityBoost_{\party^*}=z\Big|\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party\Big]+\\
&\quad+\sum_z z\cdot\Pr\Big[\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party\Big]=\\
%
&=\Big[\neg\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party\Big]\cdot\Big(\beta_\party\cdot\Pr\Big[\utilityBoost_{\party^*}=\beta_\party\Big|\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party\Big]+0\Big)+\\
&\quad+\sum_z z\cdot\negl(\secparam)\leq\\
%
&\leq\big(1-\negl(\secparam)\big)\cdot\Big(\beta_{\party^*}\cdot\Pr\Big[\utilityBoost_{\party^*}=\beta_{\party^*}\Big|\bigvee_{\party\in\partySet\setminus\{\party^*\}}F_\party\Big]+0\Big)+\big(\rounds\cdot\reward\big)^2\cdot\negl(\secparam)\leq\\
%
&\leq\big(1-\negl(\secparam)\big)\cdot\beta_{\party^*}+\negl(\secparam)=\\
%
&=\beta_{\party^*}+\negl(\secparam).
\end{split}
\end{equation}
%
Therefore, by Eq.~\eqref{eq:utility_ds_all} and~\eqref{eq:utility_ds_all_deviate}, we have that
\[\utility_{\party^*}(\profile)\leq\utility_{\party^*}(\profile_\mathsf{ds}^{\slot,\Delta})+\negl(\secparam)\;,\]
%
i.e., $\profile_\mathsf{ds}^{\slot,\Delta}$ is an $\epsilon$-Nash equilibrium  \wrt Reward under $\adversary$, for some $\epsilon=\negl(\secparam)$.\\

%----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\ref{thm:nocoor_nash2}. We have that for $\party$, $\power_\party>\frac{1}{2}$ and $\beta_\party\geq (1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\cdot\reward\cdot x$. Assume that $\party$ unilaterally deviates from $\profile_\mathsf{ds}^{\slot,\Delta}$ by following a strategy profile $\profile$. %If when following $\profile$ double-signs at any slot, then by Eq.~\eqref{eq:exchange}, it holds that $\exchangeRate_{\profile}$ is always $0$ and thus, $\utility_\party(\profile)=\beta_\party=\utility_\party(\profile_\mathsf{ds}^{\slot,\Delta})$. If $\party$ does not double sign at any round, then by  Eq.~\eqref{eq:external}, her external rewards will be $0$

Let $D$ be the event that $\party$ double-signs at some slot. If $D$ occurs, then since $\power_\party>\frac{1}{2}$ , the exchange rate will be $0$ and $\party$ will receive her external rewards. On the contrary, if $D$ does not occur, then the exchange rate will be $x$ but $\party$ will receive no external rewards. 

Let  $\msgNumber_{\party, \profile}$ be the number of blocks created by $\party$ in $\profile$. By the assumption for $\theta$ and given that $\reward_{\party, \profile}\leq\msgNumber_{\party, \profile}\cdot\reward$, we have that 
%
\begin{equation}\label{eq:utility_ds_P}
\begin{split}
\utility_\party(\profile)&=E[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}]+E[\utilityBoost_{\party, \profile}]=\sum_z z\cdot\Pr[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z]=\\
%
&=\sum_z z\cdot\Pr[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z\wedge D]+\\
&\quad+\sum_z z\cdot\Pr\big[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z\wedge \neg D\wedge\big(\msgNumber_{\party, \profile}>(1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\big)\big]+\\
&\quad+\sum_z z\cdot\Pr\big[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z\wedge \neg D\wedge\big(\msgNumber_{\party, \profile}\leq(1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\big)\big]\leq\\
%
&\leq\Pr[D]\cdot\sum_z z\cdot\Pr[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z| D]+\\
&\quad+\sum_z z\cdot\Pr\big[\msgNumber_{\party, \profile}>(1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\big]+\\
&\quad+\sum_z z\cdot\Pr\big[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z\wedge \neg D\wedge\big(\reward_{\party, \profile}\cdot \leq(1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\cdot\reward\big)\big]\leq\\
%
&\leq\Pr[D]\cdot\sum_z z\cdot\Pr[\beta_\party=z| D]+\\
&\quad+\sum_z z\cdot\Pr\big[\msgNumber_{\party, \profile_\proto}>(1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\big]+\\
&\quad+\sum_z z\cdot\Pr\big[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z\wedge \neg D\wedge\big(\reward_{\party, \profile}\cdot x\leq(1+\theta)\cdot E[\msgNumber_{\party, \profile_\proto}]\cdot\reward\cdot x\big)\big]\leq\\
%
&\leq\Pr[D]\cdot\beta_\party+(\rounds\cdot\reward)^2\cdot\negl(\secparam)+\\
&\quad+\sum_z z\cdot\Pr\big[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z\wedge \neg D\wedge\reward_{\party, \profile}\cdot x\leq\beta_\party\big]\leq\\
%
&\leq\Pr[D]\cdot\beta_\party+\negl(\secparam)+\sum_z z\cdot\Pr\big[\reward_{\party, \profile}\cdot x=z\wedge \neg D\wedge\reward_{\party, \profile}\cdot x\leq\beta_\party\big]\leq\\
%
&\leq\Pr[D]\cdot\beta_\party+\Pr[\neg D]\cdot\sum_z z\cdot\Pr\big[\reward_{\party, \profile}\cdot x=z\big|\neg D\wedge\reward_{\party, \profile}\cdot x\leq\beta_\party\big]+\negl(\secparam)=\\
%
&=\Pr[D]\cdot\beta_\party+\Pr[\neg D]\cdot\sum_{z\leq\beta_\party} z\cdot\Pr\big[\reward_{\party, \profile}\cdot x=z\big|\neg D\wedge\reward_{\party, \profile}\cdot x\leq\beta_\party\big]+\negl(\secparam)\leq\\
%
&\leq\Pr[D]\cdot\beta_\party+\Pr[\neg D]\cdot\sum_{z\leq\beta_\party} \beta\cdot\Pr\big[\reward_{\party, \profile}\cdot x=z\big|\neg D\wedge\reward_{\party, \profile}\cdot x\leq\beta_\party\big]+\negl(\secparam)=\\
%
&=\Pr[D]\cdot\beta_\party+\Pr[\neg D]\cdot\beta_\party\cdot 1+\negl(\secparam)=\beta_\party+\negl(\secparam).
\end{split}
\end{equation}
%
Besides, following the steps in Eq.~\eqref{eq:utility_ds_all}, we can show that $\utility_\party(\profile_\mathsf{ds}^{\slot,\Delta})=\beta_\party-\negl(\secparam)$. The latter along with Eq.~\eqref{eq:utility_ds_P} implies that
\[\utility_{\party}(\profile)\leq\utility_{\party}(\profile_\mathsf{ds}^{\slot,\Delta})+\negl(\secparam)\;,\]
%
i.e., $\profile_\mathsf{ds}^{\slot,\Delta}$ is an $\epsilon$-Nash equilibrium  \wrt Reward under $\adversary$, for some  $\epsilon=\negl(\secparam)$.\\


\ignore{
\vspace{100pt}
For any execution trace $\trace$, if,  when following $\profile$, the party $\party$ double-signs at any slot, then by  Eq.~\eqref{eq:exchange} and~\eqref{eq:external}, it holds that $\exchangeRate_{\profile}(\trace)=0$ and $\utilityBoost_{\party,\profile}(\trace)=\beta_\party$.  If $\party$ does not double-sign at any round, then her external rewards will be $0$ and by Eq.~\eqref{eq:exchange} and~\eqref{eq:external}, it holds that $\exchangeRate_{\profile}(\trace)=x$ and $\utilityBoost_{\party,\profile}(\trace)=0$.

Let $D$ be the event that $\party$ double-signs at some round. By the above and given that, under the synchronous router $\adversary$ and block-proportional rewards, the  (expected) ledger rewards are maximized when the parties follow $\profile_\proto$ \TZ{We have to argue about this at some point, but it seems reasonable to me}, we have that


By Eq.~\eqref{eq:utility_ds_all} and~\eqref{eq:utility_ds_P}, we get that in both Cases 1 and 2, it holds that $\utility_\party(\profile)\leq\utility_\party(\profile_\mathsf{ds}^{\slot,\Delta})$. The latter implies that $\profile_\mathsf{ds}^{\slot,\Delta}$ is a Nash equilibrium \wrt Reward.\\[2pt]
%
($\Leftarrow$) Assume that there is a party $\party $ such that $\power_\party>\frac{1}{2}$ but $\beta_\party< E[\reward_{\party, \profile_\proto}]\cdot x$. We will show that $\party$ has incentive to unilaterally deviate from $\profile_\mathsf{ds}^{\slot,\Delta}$ by behaving honestly. Let $\profile^*_\party$ be the strategy profile where $\party$ follows $\proto$ and all the other parties follow $\strategy_\mathsf{ds}^{\slot,\Delta}$. Then in $\profile^*_\party$, the exchange rate is always $x$. Moreover, by the definition of $\profile^*_\party$ and  $\strategy_\mathsf{ds}^{\slot,\Delta}$, the ledger rewards of $\party$ are equal to  $E[\reward_{\party, \profile_\proto}]$. So, we have that 
%
\[\utility_\party(\profile^*_\party)=E[\reward_{\party, \profile_\proto}]\cdot x>\beta_\party=\utility_\party(\profile_\mathsf{ds}^{\slot,\Delta})\;,\]
%
which implies that $\profile_\mathsf{ds}^{\slot,\Delta}$ is not a Nash equilibrium \wrt Reward.\\
}

%----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\ref{thm:nocoor_compliance}. Let $\party$ be a party such that $\power_\party\leq\frac{1}{2}$ and $\beta_\party>\big( E[\msgNumber_{\party, \profile_\proto}^\Delta]+1\big)\cdot\reward\cdot x$. In any unilateral deviation of $\party$ from $\profile_\proto$, since $\power_\party\leq\frac{1}{2}$ and the other parties honestly follow the protocol, it holds that the exchange rate remains always $x$. 

Assume that $\party$ unilaterally deviates from $\profile_\proto$ by following $\strategy_\mathsf{ds}^{\slot,\Delta}$, for some slot $\slot$. Let $\profile^*$ be the resulting strategy profile where all parties are honest except from $\party^*$ that follows $\strategy_\mathsf{ds}^{\slot,\Delta}$. 

Given that we utilize block-proportional rewards, we define the following random variables. Let $\reward_{\party, \profile^*}^{\slot,\Delta}$ be the ledger rewards of $\party$ when following $\profile^*$ in the time frame $[\slot,\slot+\Delta]$. Let $\overline{\reward_{\party, \profile^*}^{\slot,\Delta}}$ be the ledger rewards of $\party$ when following $\profile^*$ outside $[\slot,\slot+\Delta]$. Similarly, we define the random variables
$\reward_{\party, \profile_\proto}^{\slot,\Delta}$,  $\overline{\reward_{\party, \profile_\proto}^{\slot,\Delta}}$ for the all honest strategy profile. Since (i) throughout the execution, $\party$ creates blocks exactly as an honest party does, and (ii) within $[\slot,\slot+\Delta]$ no more than $\msgNumber_{\party, \profile_\proto}^\Delta$ blocks of $\party$ can be included in the chain of $\observer$, we have that 
\begin{equation}\label{eq:utility_ds_comp_equal}
\begin{split}
\reward_{\party, \profile^*}^{\slot,\Delta}&\leq\msgNumber_{\party, \profile_\proto}^\Delta\cdot R\\
\overline{\reward_{\party, \profile^*}^{\slot,\Delta}}&=\overline{\reward_{\party, \profile_\proto}^\Delta}\\
E[\reward_{\party, \profile_\proto}]&=E[\reward_{\party, \profile_\proto}^{\slot,\Delta}]+E[\overline{\reward_{\party, \profile_\proto}^{\slot,\Delta}}]
\end{split}
\end{equation}
%
In any execution trace $\trace$ where $\party$ follows $\profile^*$, double-signing may cause that (in the worst case) all the blocks created by $\party$ during $[\slot,\slot+\Delta]$ will not be included in $\chain_{\observer,\trace}$. However, if $\party$ double-signs, then she will get her external rewards. Hence,  the payoff of $\party$ in $\trace$ for the time frame $[\slot,\slot+\Delta]$ can be lower bounded by $\beta_\party$, if $\neg F_\party$ happens, and by  $0$, otherwise (i.e., when $\reward_{\party, \profile^*}^{\slot,\Delta}(\trace)=0$). %Thus, the payoff of $\party$ in $\trace$ can be lower bounded by $\overline{\msgNumber_{\party, \profile^*}^{\slot,\Delta}}(\trace)\cdot\reward\cdot x+\beta_\party$, if $\neg F_\party$ happens, and by  $\overline{\msgNumber_{\party, \profile^*}^{\slot,\Delta}}(\trace)\cdot\reward\cdot x$, otherwise.
%
Thus, the expected payoff of $\party$ for the time frame $[\slot,\slot+\Delta]$ can be lower bounded by 
\begin{equation*}
\begin{split}
\sum_z z\cdot\Pr[\neg F_\party]\cdot\Pr[\beta_\party=z]+\sum_z z\cdot\Pr[\neg F_\party]\cdot\Pr[0=z]=(1-q_\party^{\slot,\Delta})\cdot\beta_\party+0=\beta_\party-\negl(\secparam).
\end{split}
\end{equation*}
%
Outside $[\slot,\slot+\Delta]$, $\party$ behaves exactly as an honest party (it follows the longest chain), so the blocks she creates are added to the chain of $\observer$. Therefore, the expected payoff for the periods before and after $[\slot,\slot+\Delta]$ is equal to $E[\overline{\reward_{\party, \profile^*}^{\slot,\Delta}}]\cdot\reward\cdot x$. Overall, the utility of  $\party$ can be lower bounded as
%
\begin{equation}\label{eq:utility_ds_comp_1}
\begin{split}
\utility_{\party}(\profile^*)\geq\beta_\party-\negl(\secparam)+E[\overline{\reward_{\party, \profile^*}^{\slot,\Delta}}]\cdot x.
\end{split}
\end{equation}
%
By Eq.~\eqref{eq:utility_ds_comp_equal} and~\eqref{eq:utility_ds_comp_1} and the assumption that  $\beta_\party\geq( E[\msgNumber_{\party, \profile_\proto}^\Delta]+1)\cdot\reward\cdot x$, we have that for every $0\leq\epsilon\leq\beta_\party-( E[\msgNumber_{\party, \profile_\proto}^\Delta]+1)\cdot\reward\cdot x$
%
\begin{equation}\label{eq:utility_ds_comp_2}
\begin{split}
\utility_{\party}(\profile^*)&\geq \Big((E[\msgNumber_{\party, \profile_\proto}^\Delta]+1)\cdot\reward\cdot x+\epsilon-\negl(\secparam)\Big)+E[\overline{\reward_{\party, \profile^*}^{\slot,\Delta}}]\cdot x=\\
%
&=\Big(E[\msgNumber_{\party, \profile_\proto}^\Delta]\cdot\reward+E[\overline{\reward_{\party, \profile^*}^{\slot,\Delta}}]\Big)\cdot x+\epsilon+\reward\cdot x-\negl(\secparam)>\\
%
&>\Big(E[\msgNumber_{\party, \profile^*}^{\slot,\Delta}]\cdot\reward+E[\overline{\reward_{\party, \profile^*}^{\slot,\Delta}}]\Big)\cdot x+\epsilon\geq\\
%
&\geq\Big(E[\reward_{\party, \profile_\proto}^{\slot,\Delta}]+E[\overline{\reward_{\party, \profile_\proto}^{\slot,\Delta}}]\Big)\cdot x+\epsilon=\\
%
&=E[\reward_{\party, \profile_\proto}]\cdot x+0+\epsilon=E[\reward_{\party, \profile_\proto}\cdot\exchangeRate_{\profile_\proto}]+E[\utilityBoost_{\party, \profile_\proto}]+\epsilon=\utility_{\party}+\epsilon(\profile_\proto)
\end{split}
\end{equation}
%
Next, we show that for any unilateral deviation $\profile$ of $\party$ from the all honest profile, if $\profile$ is $\infractionPredicate_\mathsf{ds}$-compliant (i.e., $\party$ deviates from $\profile_\proto$ but never double-signs), it holds that $\utility_{\party}(\profile)\leq \utility_{\party}(\profile_\proto)$. The latter holds because (i)   the expected ledger rewards are maximized in $\profile_\proto$, i.e., $E[\reward_{\party, \profile}]\leq E[\reward_{\party, \profile_\proto}]$; (ii) since $\infractionPredicate_\mathsf{ds}$-compliant, the external rewards of $\party$ in $\profile$ are always $0$. Consequently, if there is a best response for $\party$ with strictly greater utility than of $\profile_\proto$, then it must be not $\infractionPredicate_\mathsf{ds}$-compliant.

By the above, the fact that  $\profile^*$ is not $\infractionPredicate_\mathsf{ds}$-compliant, and Eq.~\eqref{eq:utility_ds_comp_2}, we conclude that there is a strategy profile $\profile_\mathsf{best}$ (not necessarily $\profile^*$) that (i) is a unilateral deviation from $\profile_\proto$, (ii) $\utility_{\party}(\profile_\mathsf{best})> \utility_{\party}(\profile_\proto)+\epsilon$, (iii) sets a best response for $\party$ 
, and (iv) not $\infractionPredicate_\mathsf{ds}$-compliant. 

So, for every $0\leq\epsilon\leq\beta_\party-( E[\msgNumber_{\party, \profile_\proto}^\Delta]+1)\cdot\reward\cdot x$, $\profile_\mathsf{best}$ is directly $\epsilon$-reachable from $\profile_\proto$ which implies that $\proto$ is not $(\epsilon,\infractionPredicate_\mathsf{ds})$-compliant \wrt Reward under $\adversary$.\\

%----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\ref{thm:nocoor_reachable}. Assume that $\beta_\party> E[\reward_{\party, \profile_\proto}]\cdot x$ for every party $\party\in\partySet$.  Let $\profile_j^{\slot,\Delta}$, $j\in\{0,\ldots,n\}$ be the strategy profile where parties $\party_1,\ldots,\party_j$ follow $\strategy_\mathsf{ds}^{\slot,\Delta}$ while the parties $\party_{j+1},\ldots,\party_n$ follow $\Pi$. Clearly (i) $\profile_0^\slot=\profile_\proto$, (ii) $\profile_n^{\slot,\Delta}=\profile_\mathsf{ds}^{\slot,\Delta}$, and (iii)  for every $j\in\{1,\ldots,n\}$, $\profile_j^{\slot,\Delta}$, $\profile_j^{\slot,\Delta}$ is a unilateral deviation of $\party_j$ from $\profile_{j-1}^\slot$. Therefore, it suffices to show that  for every $j\in\{1,\ldots,n\}$, $\utility_{\party_j}(\profile_j^{\slot,\Delta})> \utility_{\party_j}(\profile_{j-1}^{\slot,\Delta})$.

%We observe that (a) when parties all honest, the exchange rate is always $x$ and the parties' external rewards are always 0; (b) by following  $\strategy_\mathsf{ds}^{\slot,\Delta}$, the parties' expected number of blocks (hence, their ledger rewards) is not affected compared to they being honest, i,.e., $E[\reward_{\party, \profile_1^\slot}]=\cdots=E[\reward_{\party, \profile_n^\slot}]=E[\reward_{\party, \profile_\proto}]$. We study the following cases: 
For every $j\in\{0,\ldots,n\}$, we define the following random variables. Let $\reward_{\party_j,j}^{\slot,\Delta}$ (resp. $\reward_{\party_j,{j-1}}^{\slot,\Delta}$) be the ledger rewards of $\party_j$ when following $\profile_j^{\slot,\Delta}$ (resp.  $\profile_{j-1}^{\slot,\Delta}$)  in the time frame $[\slot,\slot+\Delta]$. Let $\overline{\reward_{\party_j,j}^{\slot,\Delta}}$ (resp. $\reward_{\party_j,{j-1}}^{\slot,\Delta}$) be the ledger rewards of $\party_j$ when following $\profile_j^{\slot,\Delta}$ (resp.  $\profile_{j-1}^{\slot,\Delta}$) outside $[\slot,\slot+\Delta]$. 

We observe that
\begin{enumerate}[(i).]
\item In the time frame $[\slot,\slot+\Delta]$, the ledger rewards of $\party_j$ could be reduced due to double signing, as her blocks may not be added in the chain  not only due to concurrent mining but because the other parties may not follow the fork that $\party_j$ creates. Formally, for every execution trace $\trace$, $\reward_{\party_j,j}^{\slot,\Delta}(\trace)\leq\reward_{\party_j,j-1}^{\slot,\Delta}(\trace)$.
%
\item Outside $[\slot,\slot+\Delta]$, $\party_j$ behaves just as an honest party following the longest chain, so for every every execution trace $\trace$, $\overline{\reward_{\party_j,j}^{\slot,\Delta}}(\trace)=\overline{\reward_{\party_j,j-1}^{\slot,\Delta}}(\trace)$.
%
\item For every execution trace $\trace$, the maximum blocks of $\party_j$ that can in be included in the chain of $\observer$ is $\msgNumber_{\party_j, \profile_\proto}(\trace)$. So, $\reward_{\party_j, \profile_\proto}(\trace)\leq\msgNumber_{\party_j, \profile_\proto}(\trace)\cdot\reward$.
\end{enumerate}
 %
Based on the above three observations, we study the following cases:

\emph{Case 1}:  By unilaterally deviating from  $\profile_{j-1}^{\slot,\Delta}$ to  $\profile_j^{\slot,\Delta}$, the party $\party_j$'s double-signing  does not affect the exchange rate. In this case, $\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}=\exchangeRate_{\profile_j^{\slot,\Delta}}$. In addition, unless $F_{\party_j}$ happens (with $\negl(\secparam)$ probability), $\party_j$ will receive her external rewards. Thus, in this case,  since $\beta_{\party_j}> \big(E[\reward_{\party_j, \profile_\proto}]+1\big)\cdot x$, we have that for every $0\leq\epsilon\leq\beta_{\party_j}-\big(E[\msgNumber_{\party_j, \profile_\proto}]\cdot\reward+1\big)\cdot x$,
\begin{equation*}
\begin{split}
\utility_{\party_j}(\profile_j^{\slot,\Delta})&=E[\reward_{\party_j, \profile_j^{\slot,\Delta}}\cdot\exchangeRate_{\profile_j^{\slot,\Delta}}]+E[\utilityBoost_{\party_j, \profile_j^{\slot,\Delta}}]\geq E[\overline{\reward_{\party_j,j}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_j^{\slot,\Delta}}]+(1-\Pr[F_{\party_j}])\cdot\beta_{\party_j}=\\
%
&=E[\overline{\reward_{\party_j,j-1}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}]+\beta_{\party_j}-\negl(\secparam)\geq\\
%
&\geq E[\overline{\reward_{\party_j,j-1}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}]+\big(E[\msgNumber_{\party_j, \profile_\proto}]\cdot\reward+1\big)\cdot x+\epsilon-\negl(\secparam)\geq\\
%
&\geq E[\overline{\reward_{\party_j,j-1}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}]+\big(E[\reward_{\party_j, \profile_\proto}]+1\big)\cdot x+\epsilon-\negl(\secparam)\geq\\
%
&\geq E[\overline{\reward_{\party_j,j-1}^{\slot,\Delta}}]\cdot x+E[\reward_{\party_j,j-1}^{\slot,\Delta}]\cdot x+\epsilon+x-\negl(\secparam)\geq\\
%
&\geq E[\overline{\reward_{\party_j,j-1}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}]+E[\reward_{\party_j,j-1}^{\slot,\Delta}]\cdot x+\epsilon+x-\negl(\secparam)\geq\\
%
&\geq E[\overline{\reward_{\party_j,j-1}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}]+E[\reward_{\party_j,j-1}^{\slot,\Delta}\cdot\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}]+\epsilon+x-\negl(\secparam) > \\
%
&>E[\reward_{\party_j, \profile_{j-1}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}]+\epsilon=\utility_{\party_j}(\profile_{j-1}^{\slot,\Delta})+\epsilon.
\end{split}
\end{equation*}
%
%On the other hand, if the rate in both strategy profiles is $0$, this means that $\utility_\party(\profile_{j-1}^\slot)=0$, so $\party$ has incentive to act like $\party_1,\cdots,\party_{j-1}$ and double sign in $\slot$ in order to gain positive external rewards $\beta_\party$. So, $\utility_\party(\profile_j^\slot)-\beta_\party>0=\utility_\party(\profile_{j-1}^\slot)$
\indent\emph{Case 2}:  By unilaterally deviating from  $\profile_{j-1}^{\slot,\Delta}$ to  $\profile_j^{\slot,\Delta}$, the party $\party_j$'s double-signing affects the exchange rate. In this case the rate, unless $F_{\party_j}$ happens, $\party_j$ at least gets her external rewards. Thus, for every $0\leq\epsilon\leq\beta_{\party_j}-\big(E[\msgNumber_{\party_j, \profile_\proto}]\cdot\reward+1\big)\cdot x$,
\begin{equation*}
\begin{split}
\utility_{\party_j}(\profile_j^{\slot,\Delta})&\geq E[\utilityBoost_{\party_j, \profile_j^{\slot,\Delta}}]= (1-\Pr[F_{\party_j}])\cdot\beta_{\party_j}=\beta_{\party_j}-\negl(\secparam)\geq\\
%
&\geq \big(E[\reward_{\party_j, \profile_\proto}]+1\big)\cdot x+\epsilon-\negl(\secparam)\geq E[\reward_{\party_j, \profile_{j-1}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}]+\epsilon+ x-\negl(\secparam)\geq\\
%
&\geq E[\reward_{\party_j, \profile_{j-1}^{\slot,\Delta}}]\cdot x+\epsilon+ x-\negl(\secparam)>E[\reward_{\party_j, \profile_{j-1}^{\slot,\Delta}}\cdot\exchangeRate_{\profile_{j-1}^{\slot,\Delta}}]+\epsilon=\utility_{\party_j}(\profile_{j-1}^{\slot,\Delta})+\epsilon.
%
\end{split}
\end{equation*}
%
Therefore, in both  Cases 1 and 2, it holds that $\utility_{\party_j}(\profile_j^{\slot,\Delta})> \utility_{\party_j}(\profile_{j-1}^{\slot,\Delta})$, for every $j\in[n]$. Thus, for every $0\leq\epsilon\leq\underset{j\in[n]}{\mathsf{min}}\big\{\beta_{\party_j}-\big(E[\msgNumber_{\party_j, \profile_\proto}]\cdot\reward+1\big)\cdot x\big\}$, $\profile_j^\slot$ is weakly directly $\epsilon$-reachable from $\profile_\proto$ \wrt Reward under $\adversary$.\TZ{Maybe we do not need to study cases. The analysis in Case 2 seems to work for Case 2 as well. }


\ignore{
3. To show that $\strategy_\mathsf{ds}^{\slot,\Delta}$ is a dominant strategy, assume that the parties follow some strategy $\profile$ such that the party $\party$ follows $\strategy_\mathsf{ds}^{\slot,\Delta}$ and a unilaterally deviation from $\profile$ to $\profile'$ because $\party$ decided to follow some strategy $\strategy'\neq\strategy_\mathsf{ds}^{\slot,\Delta}$. We will prove that $\utility_\party(\profile)>\utility_\party(\profile')$.

Let $D$ be the event that $\party$ double-signs at some round when following $\strategy'$. For every trace $\trace$ \wrt $\profile'$, if $D$ does not happen, then the payoff of $\party$ is  upper bounded by $\reward_{\party, \profile}(\trace)\cdot x$ (recall that the rate can be either $x$ or $0$). Otherwise, the payoff of $\party$ is lower bounded by her external rewards $\beta_\party$. Thus, we have that

\begin{equation}\label{eq:dominant}
\begin{split}
&\utility_\party(\profile')=\sum_z z\cdot\Pr[\reward_{\party, \profile'}\cdot\exchangeRate_{\profile'}+\utilityBoost_{\party, \profile'}=z]=\sum_z z\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)+\utilityBoost_{\party, \profile'}(\trace)=z}\Pr[\trace]=\\
%
=&\sum_z z\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)+\utilityBoost_{\party, \profile'}(\trace)=z\wedge D}\Pr[\trace]+\sum_z z\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)+\utilityBoost_{\party, \profile'}(\trace)=z\wedge\neg D}\Pr[\trace]=\\
%
=&\beta_\party\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)+\utilityBoost_{\party, \profile'}(\trace)=\beta_\party\wedge D}\Pr[\trace]+\sum_z z\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)=z\wedge\neg D}\Pr[\trace]
\end{split}
\end{equation}
}

\end{proof}

\begin{remark}
Given the results of Theorem~\ref{thm:nocoor}, it is reasonable to ask whether $\strategy_\mathsf{ds}^{\slot,\Delta}$ is also a dominant strategy. However,  a simple counterexample shows that this is not the case. Consider the scenario where by double-signing at slot $\slot$, some party $\party$ with $\power_\party\leq\frac{1}{2}$ causes the exchange rate to drop from $x$ to $0$. Then, it is profitable for  $\party$ to perform double-signing at some other round, say, $r+1$, so that the exchange rate remains $x$, yet $\party$ will still get her external rewards $\beta_\party$. In other words, $\party$ exploits the fact that coordination is not necessary for the parties to get their external reward.\TZ{Even in coordination it is hard to show dominance. The reason is that in general (e.g. in PoW), the briber cannot verify whether the party has created one block or more. Thus, the briber cannot force the parties to support the fork they create by double-signing with many blocks. In Ouroboros, however the number of blocks that a party should contribute as slot leader is verifiable.}

 Interestingly, the above counterexample indicates something stronger. Namely, that  $\profile_\mathsf{ds}^{\slot,\Delta}$ is not reachable from the all honest strategy profile $\profile_\proto$. This is formally shown in the proposition below.\TZ{Hmmm not that easy. There are complex strategies e.g., $\party_i$ double-signs in $\slot$ only if $\party_j$ does not double-sign. I do not know how to prove this proposition below.}
\end{remark}

\begin{proposition}\label{prop:nocoor}
Let $\proto$ be a protocol with block-proportional rewards (cf. Subsection~\ref{subsec:preliminaries_proportion}) with $\reward$ rewards per block. Let $\profile_\proto$ denote the all-honest strategy profile. Assume that for any strategy profile $\sigma$, the exchange rate $\exchangeRate_\profile$ is defined as in Eq.~\eqref{eq:exchange} and the external rewards $\utilityBoost_{\party,\profile}$ due to non-coordinated bribing are defined as in Eq.~\eqref{eq:external}. Let $\adversary$ be a synchronous router. Then, it holds that  for every slot $\slot$, $\profile_\mathsf{ds}^{\slot,\Delta}$ is not reachable from $\profile_\proto$ \wrt Reward under $\adversary$.
\end{proposition}
\ignore{
\begin{proof}
For the sake of contradiction, assume that for some slot $\slot$, $\profile_\mathsf{ds}^{\slot,\Delta}$ is reachable from $\profile_\proto$ via a path of directly reachable strategy profiles $\profile_\proto=\profile_1\longrightarrow\profile_2\longrightarrow\cdots\longrightarrow\profile_k=\profile_\mathsf{ds}^{\slot,\Delta}$ (here, $k\geq\totalParties$). We observe that
\begin{enumerate}[(a)]
\item in $\profile_\proto$, the exchange rate is always $x$ and the condition $\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}$ never holds,
\item in $\profile_\mathsf{ds}^{\slot,\Delta}$, the exchange is always $0$ because the condition $\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}$ always holds.
\end{enumerate}
 This implies that there is $j^*\in[k-1]$ such that the condition  $\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}$ always holds in $\profile_{j^*+1}$ but with some probability $q>0$, the condition $\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}$ does not hold in $\profile_{j^*}$. Let $\party^*$ be the party that unilaterally deviates from $\profile_{j^*+1}$ to $\profile_{j^*}$.
\end{proof}
}


==> sections/bribing_toy.tex <==
\section{Equilibria under bribing attacks}\label{sec:bribing}

\subsection{A toy example}\label{subsec:bribing_toy}
Let the parties $\party_1,\ldots\party_\totalParties$ follow strategy profile $\profile=\langle\strategy_1,\ldots,\strategy_\totalParties\rangle$ and that no party has participation power $>\frac{1}{2}$. The parties adaptively decide whether to double-sign at some point in the execution. Let the exchange rate  be defined as follows:
%
\begin{equation}\label{eq:toy_exchange}
\exchangeRate_\profile(\trace)=\left\{\begin{array}{ll}x,&\mbox{if in $\trace$, for every slot }\slot:\sum_{\party: \party\text{ double-signs in }\slot}\power_\party\leq\frac{1}{2}\\
0,&\mbox{if in $\trace$, there is a slot }\slot:\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}\end{array}\right.\;,
\end{equation}
%
where $x$ is some positive constant. Namely, we assume an extreme token toxicity effect where the ledger token's price goes to $0$.\TZ{In Eq.~\eqref{eq:toy_exchange}, I tried to capture the fact that there is a condition such that the exchange rate drops to $0$. If you think that this condition is not realistic, we can change it, I do not think the analysis will be much affected.}

We define the \emph{double-signing} infraction predicate as follows. For every execution trace $\trace$ and party $\party\in\partySet$:

\begin{equation}\label{eq:infraction_ds}
\infractionPredicate_\mathsf{ds}(\trace,\party)=\left\{\begin{array}{ll}1,& \mbox{if in $\trace$, there is a slot }\slot: \party\mbox{ double-signs in }\slot\\
0,&\mbox{otherwise}\end{array}\right.\;,
\end{equation}

We define the strategy $\strategy_\mathsf{ds}^\slot$ as follows: the party behaves honestly throughout the execution, except that it double-signs in slot $\slot$. The strategy profile where all parties double-sign in $\slot$ is denoted by $\profile_\mathsf{ds}^\slot=\langle\strategy_\mathsf{ds}^\slot,\ldots,\strategy_\mathsf{ds}^\slot\rangle$.


\subsubsection{Non-coordinated bribing attacks}\label{subsubsec:bribing_toy_nocoor}
In the non-coordinated setting, the briber tempts the parties to double-sign by offering them an amount of external rewards if they do at any preferred moment. This is formalized as follows: %\TZ{We do not need to define the external rewards \wrt some specific slot $\slot$. Coordination of the parties regarding when they double sign is specified by the strategy profile.}

\begin{equation}\label{eq:toy_external}
\utilityBoost_{\party,\profile}(\trace)=\left\{\begin{array}{ll}\beta_\party,& \mbox{if in $\trace$, there is a slot }\slot: \party\mbox{ double-signs in }\slot\\
0,&\mbox{otherwise}\end{array}\right.\;,
\end{equation}
%
where $\beta_\party$ is some positive constant.  

In the following theorem, we prove that under non-coordinated bribing, a synchronous network and the Reward utility function:
\begin{enumerate}
\item  $\strategy_\mathsf{ds}^\slot$ is a Nash equilibrium if the protocol is decentralized.

\item  $\strategy_\mathsf{ds}^\slot$ is an approximate Nash equilibrium if the protocol it is centralized, but the bribe for the party that holds the majority of participation power is sufficiently large (it exceeds the expected system's rewards).
%
\item The protocol $\proto$ is not  $\infractionPredicate_\mathsf{ds}$-compliant.
%
\item  $\strategy_\mathsf{ds}^\slot$ is weakly reachable from the all honest strategy profile under the stronger condition that the bribe for all parties is sufficiently large.\TZ{By ``weakly'' I mean that the players do not move only to best responses. If this result makes sense, we can add the definition of ``weak'' reachability.}
\end{enumerate}

\begin{theorem}\label{thm:toy_nocoor}
Let $\proto$ be a protocol with block-proportional rewards (cf. Subsection~\ref{subsec:preliminaries_proportion}) with $\reward$ rewards per block. Let $\profile_\proto$ denote the all-honest strategy profile. Assume that for any strategy profile $\sigma$, the exchange rate $\exchangeRate_\profile$ is defined as in Eq.~\eqref{eq:toy_exchange} and the external rewards $\utilityBoost_{\party,\profile}$ due to non-coordinated bribing are defined as in Eq.~\eqref{eq:toy_external}. Let $\adversary$ be a synchronous router. Then, the following hold:
%
\begin{enumerate}
%\item\label{thm:toy_nocoor_nash} For every slot $\slot$, the strategy profile  $\profile_\mathsf{ds}^\slot$ is a Nash equilibrium \wrt Reward under $\adversary$.$\forall\party\in\partySet:\big(\power_\party>\frac{1}{2}\Rightarrow\beta_\party\geq E[\reward_{\party, \profile_\proto}]\cdot x\big)$ if and only if 
\item\label{thm:toy_nocoor_nash1} If for every party $\party\in\partySet$, it holds that $\power_\party\leq\frac{1}{2}$, then the strategy profile  $\profile_\mathsf{ds}^\slot$ is a Nash equilibrium \wrt Reward under $\adversary$.\TZ{Completed}
%
\item\label{thm:toy_nocoor_nash2}  If there is a (unique) party $\party$ such that $\power_\party>\frac{1}{2}\wedge\beta_\party\geq E[\reward_{\party, \profile_\proto}]\cdot x$ holds, then the strategy profile  $\profile_\mathsf{ds}^\slot$ is an $\epsilon$-Nash equilibrium \wrt Reward under $\adversary$, where $\epsilon$ is $\mathsf{negl}(\secparam)$.\TZ{This is very tricky and the proof is pending. There are complex strategies like ``if I have produced less than the expected number of blocks up to $\slot$, I will double sign. Otherwise, I will behave honestly''. The conditional probabilities in such cases are complete mindfuck.}
%
\item\label{thm:toy_nocoor_compliance} $\proto$ is not $\infractionPredicate_\mathsf{ds}$-compliant \wrt Reward under $\adversary$.\TZ{Completed}
%
\item\label{thm:toy_nocoor_reachable} If $\beta_\party> E[\reward_{\party, \profile_\proto}]\cdot x$ for every party $\party\in\partySet$, then for every slot $\slot$,  $\profile_\mathsf{ds}^\slot$ is weakly reachable from $\profile_\proto$ \wrt Reward under $\adversary$.\TZ{Completed}
\end{enumerate}
\end{theorem}

\begin{proof}
\ref{thm:toy_nocoor_nash1}. ($\Rightarrow$) Assume that the parties follow $\profile_\mathsf{ds}^\slot=\langle\strategy_\mathsf{ds}^\slot,\ldots,\strategy_\mathsf{ds}^\slot\rangle$. Then, by Eq.~\eqref{eq:toy_exchange} and~\eqref{eq:toy_external}, the utility of some party $\party$ is 
\begin{equation}\label{eq:toy_utility_ds_all}
\utility_\party(\profile_\mathsf{ds}^\slot)=E[\reward_{\party, \profile_\mathsf{ds}^\slot}\cdot\exchangeRate_{\profile_\mathsf{ds}^\slot}]+E[\utilityBoost_{\party, \profile_\mathsf{ds}^\slot}]=E[\reward_{\party, \profile_\mathsf{ds}^\slot}]\cdot 0+\beta_\party=\beta_\party.
\end{equation}
Assume now that some party $\party$ unilaterally deviates from $\profile_\mathsf{ds}^\slot$ to some strategy profile $\profile$. We study the following cases.

%Below, we show that $\utility_\party(\profile_\mathsf{ds}^\slot)$ is the maximum for the utility of $\party$
%\emph{Case 1}:  $\power_\party\leq\frac{1}{2}$. Observe that  all other parties, which sum of participation powers is greater than $\frac{1}{2}$, double-sign in $\slot$ when following $\profile$. Therefore, by Eq.~\eqref{eq:toy_exchange}, it holds that $\exchangeRate_{\profile}$ is always $0$ and thus, $\utility_\party(\profile)=\beta_\party=\utility_\party(\profile_\mathsf{ds}^\slot)$.
By assumption, $\power_\party\leq\frac{1}{2}$. Observe that  all other parties, which sum of participation powers is greater than $\frac{1}{2}$, double-sign in $\slot$ when following $\profile$. Therefore, by Eq.~\eqref{eq:toy_exchange}, it holds that $\exchangeRate_{\profile}$ is always $0$ and thus, $\utility_\party(\profile)\leq\beta_\party=\utility_\party(\profile_\mathsf{ds}^\slot)$.\\

\ref{thm:toy_nocoor_nash2}. We have that for $\party$, $\power_\party>\frac{1}{2}$ and $\beta_\party\geq E[\reward_{\party, \profile_\proto}]\cdot x$.  %If when following $\profile$ double-signs at any slot, then by Eq.~\eqref{eq:toy_exchange}, it holds that $\exchangeRate_{\profile}$ is always $0$ and thus, $\utility_\party(\profile)=\beta_\party=\utility_\party(\profile_\mathsf{ds}^\slot)$. If $\party$ does not double sign at any round, then by  Eq.~\eqref{eq:toy_external}, her external rewards will be $0$
For any execution trace $\trace$, if,  when following $\profile$, the party $\party$ double-signs at any slot, then by  Eq.~\eqref{eq:toy_exchange} and~\eqref{eq:toy_external}, it holds that $\exchangeRate_{\profile}(\trace)=0$ and $\utilityBoost_{\party,\profile}(\trace)=\beta_\party$.  If $\party$ does not double-sign at any round, then her external rewards will be $0$ and by Eq.~\eqref{eq:toy_exchange} and~\eqref{eq:toy_external}, it holds that $\exchangeRate_{\profile}(\trace)=x$ and $\utilityBoost_{\party,\profile}(\trace)=0$.

Let $D$ be the event that $\party$ double-signs at some round. By the above and given that, under the synchronous router $\adversary$ and block-proportional rewards, the  (expected) ledger rewards are maximized when the parties follow $\profile_\proto$ \TZ{We have to argue about this at some point, but it seems reasonable to me}, we have that
\begin{equation}\label{eq:toy_utility_ds_P}
\begin{split}
&\utility_\party(\profile)=E[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}]+E[\utilityBoost_{\party, \profile}]=\sum_z z\cdot\Pr[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z]=\\
%
=&\sum_z z\cdot\big(\Pr[D]\cdot\Pr[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z\mid D]+\Pr[\neg D]\cdot\Pr[\reward_{\party, \profile}\cdot\exchangeRate_{\profile}+\utilityBoost_{\party, \profile}=z\mid \neg D]\big)=\\
%
&\mbox{\TZ{here the proof breaks :(}}\\
%
=&\Pr[D]\cdot\sum_z z\cdot\Pr[\reward_{\party, \profile}\cdot 0+\beta_\party=z]+\Pr[\neg D]\cdot\sum_z z\cdot\Pr[\reward_{\party, \profile}\cdot x+0=z]=\\
%
=&\Pr[D]\cdot\beta_\party+\Pr[\neg D]\cdot E[\reward_{\party, \profile}\cdot x]\leq\mathsf{max}\{\beta_\party,E[\reward_{\party, \profile}]\cdot x\}\leq\mathsf{max}\{\beta_\party,E[\reward_{\party, \profile_\proto}]\cdot x\}=\beta_\party=\\=&\utility_\party(\profile_\mathsf{ds}^\slot).
\end{split}
\end{equation}

By Eq.~\eqref{eq:toy_utility_ds_all} and~\eqref{eq:toy_utility_ds_P}, we get that in both Cases 1 and 2, it holds that $\utility_\party(\profile)\leq\utility_\party(\profile_\mathsf{ds}^\slot)$. The latter implies that $\profile_\mathsf{ds}^\slot$ is a Nash equilibrium \wrt Reward.\\[2pt]
%
($\Leftarrow$) Assume that there is a party $\party $ such that $\power_\party>\frac{1}{2}$ but $\beta_\party< E[\reward_{\party, \profile_\proto}]\cdot x$. We will show that $\party$ has incentive to unilaterally deviate from $\profile_\mathsf{ds}^\slot$ by behaving honestly. Let $\profile^*_\party$ be the strategy profile where $\party$ follows $\proto$ and all the other parties follow $\strategy_\mathsf{ds}^\slot$. Then in $\profile^*_\party$, the exchange rate is always $x$. Moreover, by the definition of $\profile^*_\party$ and  $\strategy_\mathsf{ds}^\slot$, the ledger rewards of $\party$ are equal to  $E[\reward_{\party, \profile_\proto}]$. So, we have that 
%
\[\utility_\party(\profile^*_\party)=E[\reward_{\party, \profile_\proto}]\cdot x>\beta_\party=\utility_\party(\profile_\mathsf{ds}^\slot)\;,\]
%
which implies that $\profile_\mathsf{ds}^\slot$ is not a Nash equilibrium \wrt Reward.\\

\ref{thm:toy_nocoor_compliance}. Let $\party^*$ be a party such that $\power_{\party^*}\leq\frac{1}{2}$ (such a party always exists). Assume that $\party^*$ unilaterally deviates from $\profile_\proto$ by following $\strategy_\mathsf{ds}^\slot$, for some slot $\slot$. Let $\profile^*$ be the resulting strategy profile where all parties are honest except from $\party^*$ that follows $\strategy_\mathsf{ds}^\slot$. 

As in $\profile_\proto$, it holds that the exchange rate is always $x$ in $\profile^*$. The reason is that since $\power_{\party^*}\leq\frac{1}{2}$, even if $\party^*$ double-signs, then honest behavior of all the other  parties ensures that the condition $\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}$ will never be met.
 In addition, in both strategy profiles the expected ledger rewards are maximized and equal to $E[\reward_{\party^*, \profile^*}]=E[\reward_{\party^*, \profile_\proto}]$ (the expected number of parties' blocks remains unaffected when $\party^*$ follows $\strategy_\mathsf{ds}^\slot$). As a result, the utility of $\party^*$ is maximized in $\profile^*$ as $\utility_{\party^*}(\profile^*)=E[\reward_{\party^*, \profile_\proto}]\cdot x+\beta_{\party^*}$. 

Clearly, $\utility_{\party^*}(\profile^*)>E[\reward_{\party^*, \profile_\proto}]\cdot x=\utility_{\party^*}(\profile_\proto)$, i.e. $\profile^*$ is directly reachable from $\profile_\proto$. In addition,  $\profile^*$ sets a best response for $\party^*$. Since $\profile^*$ is not $\infractionPredicate_\mathsf{ds}$-compliant, we conclude that $\proto$ is not $\infractionPredicate_\mathsf{ds}$-compliant \wrt Reward.\\


\ref{thm:toy_nocoor_reachable}. Assume that $\beta_\party> E[\reward_{\party, \profile_\proto}]\cdot x$ for every party $\party\in\partySet$.  Let $\profile_j^\slot$, $j\in\{0,\ldots,n\}$ be the strategy profile where parties $\party_1,\ldots,\party_j$ follow $\strategy_\mathsf{ds}^\slot$ while the parties $\party_{j+1},\ldots,\party_n$ follow $\Pi$. Clearly $\profile_0^\slot=\profile_\proto$ and $\profile_n^\slot=\profile_\mathsf{ds}^\slot$. Therefore, it suffices to show that  for every $j\in\{1,\ldots,n\}$, $\profile_j^\slot$ is weakly directly reachable from $\profile_{j-1}^\slot$.

We observe that (a) when parties all honest, the exchange rate is always $x$ and the parties' external rewards are always 0; (b) by following  $\strategy_\mathsf{ds}^\slot$, the parties' expected number of blocks (hence, their ledger rewards) is not affected compared to they being honest, i,.e., $E[\reward_{\party, \profile_1^\slot}]=\cdots=E[\reward_{\party, \profile_n^\slot}]=E[\reward_{\party, \profile_\proto}]$. We study the following cases: 

\emph{Case 1}:  By unilaterally deviating from  $\profile_{j-1}^\slot$ to  $\profile_j^\slot$, the party $\party_j$'s double-signing  does not affect the exchange rate. In this case, if the rate in both strategy profiles is $c\in\{0,x\}$, then the utility of $\party_j$ becomes
\[\utility_{\party_j}(\profile_j^\slot)=E[\reward_{\party_j, \profile_j^\slot}]\cdot c+\beta_{\party_j}>E[\reward_{\party_j, \profile_{j-1}^\slot}]\cdot c+0=\utility_{\party_j}(\profile_{j-1}^\slot).\] 
%
%On the other hand, if the rate in both strategy profiles is $0$, this means that $\utility_\party(\profile_{j-1}^\slot)=0$, so $\party$ has incentive to act like $\party_1,\cdots,\party_{j-1}$ and double sign in $\slot$ in order to gain positive external rewards $\beta_\party$. So, $\utility_\party(\profile_j^\slot)-\beta_\party>0=\utility_\party(\profile_{j-1}^\slot)$
\indent\emph{Case 2}:  By unilaterally deviating from  $\profile_{j-1}^\slot$ to  $\profile_j^\slot$, the party $\party_j$'s double-signing affects the exchange rate. In this case the rate in $\profile_j^\slot$ is $x$ whereas the rate in $\profile_j^\slot$ drops to $0$. Thus, the utility of $\party_j$ becomes
\[\utility_{\party_j}(\profile_j^\slot)=\beta_{\party_j}> E[\reward_{\party_j, \profile_\proto}]\cdot x= E[\reward_{\party_j, \profile_{j-1}^\slot}]\cdot x+0=\utility_{\party_j}(\profile_{j-1}^\slot).\] 
%
Therefore, in both  Cases 1 and 2, it holds that $\utility_{\party_j}(\profile_j^\slot)> \utility_{\party_j}(\profile_{j-1}^\slot)$, i.e., $\profile_j^\slot$ is weakly directly reachable from $\profile_{j-1}^\slot$.


\ignore{
3. To show that $\strategy_\mathsf{ds}^\slot$ is a dominant strategy, assume that the parties follow some strategy $\profile$ such that the party $\party$ follows $\strategy_\mathsf{ds}^\slot$ and a unilaterally deviation from $\profile$ to $\profile'$ because $\party$ decided to follow some strategy $\strategy'\neq\strategy_\mathsf{ds}^\slot$. We will prove that $\utility_\party(\profile)>\utility_\party(\profile')$.

Let $D$ be the event that $\party$ double-signs at some round when following $\strategy'$. For every trace $\trace$ \wrt $\profile'$, if $D$ does not happen, then the payoff of $\party$ is  upper bounded by $\reward_{\party, \profile}(\trace)\cdot x$ (recall that the rate can be either $x$ or $0$). Otherwise, the payoff of $\party$ is lower bounded by her external rewards $\beta_\party$. Thus, we have that

\begin{equation}\label{eq:toy_dominant}
\begin{split}
&\utility_\party(\profile')=\sum_z z\cdot\Pr[\reward_{\party, \profile'}\cdot\exchangeRate_{\profile'}+\utilityBoost_{\party, \profile'}=z]=\sum_z z\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)+\utilityBoost_{\party, \profile'}(\trace)=z}\Pr[\trace]=\\
%
=&\sum_z z\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)+\utilityBoost_{\party, \profile'}(\trace)=z\wedge D}\Pr[\trace]+\sum_z z\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)+\utilityBoost_{\party, \profile'}(\trace)=z\wedge\neg D}\Pr[\trace]=\\
%
=&\beta_\party\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)+\utilityBoost_{\party, \profile'}(\trace)=\beta_\party\wedge D}\Pr[\trace]+\sum_z z\cdot\sum_{\trace: \reward_{\party, \profile'}(\trace)\cdot\exchangeRate_{\profile'}(\trace)=z\wedge\neg D}\Pr[\trace]
\end{split}
\end{equation}
}

\end{proof}

\begin{remark}
Given the results of Theorem~\ref{thm:toy_nocoor}, it is reasonable to ask whether $\strategy_\mathsf{ds}^\slot$ is also a dominant strategy. However,  a simple counterexample shows that this is not the case. Consider the scenario where by double-signing at slot $\slot$, some party $\party$ with $\power_\party\leq\frac{1}{2}$ causes the exchange rate to drop from $x$ to $0$. Then, it is profitable for  $\party$ to perform double-signing at some other round, say, $r+1$, so that the exchange rate remains $x$, yet $\party$ will still get her external rewards $\beta_\party$. In other words, we exploit the fact that coordination is not necessary for the parties to get their external reward.

 Interestingly, the above counterexample indicates something stronger. Namely, that  $\profile_\mathsf{ds}^\slot$ is not reachable from the all honest strategy profile $\profile_\proto$. This is formally shown in the proposition below.\TZ{Hmmm not that easy. There are complex strategies e.g., $\party_i$ double-signs in $\slot$ only if $\party_j$ does not double-sign. I do not know how to prove this proposition below.}
\end{remark}

\begin{proposition}\label{prop:toy_nocoor}
Let $\proto$ be a protocol with block-proportional rewards (cf. Subsection~\ref{subsec:preliminaries_proportion}) with $\reward$ rewards per block. Let $\profile_\proto$ denote the all-honest strategy profile. Assume that for any strategy profile $\sigma$, the exchange rate $\exchangeRate_\profile$ is defined as in Eq.~\eqref{eq:toy_exchange} and the external rewards $\utilityBoost_{\party,\profile}$ due to non-coordinated bribing are defined as in Eq.~\eqref{eq:toy_external}. Let $\adversary$ be a synchronous router. Then, it holds that  for every slot $\slot$, $\profile_\mathsf{ds}^\slot$ is not reachable from $\profile_\proto$ \wrt Reward under $\adversary$.
\end{proposition}
\ignore{
\begin{proof}
For the sake of contradiction, assume that for some slot $\slot$, $\profile_\mathsf{ds}^\slot$ is reachable from $\profile_\proto$ via a path of directly reachable strategy profiles $\profile_\proto=\profile_1\longrightarrow\profile_2\longrightarrow\cdots\longrightarrow\profile_k=\profile_\mathsf{ds}^\slot$ (here, $k\geq\totalParties$). We observe that
\begin{enumerate}[(a)]
\item in $\profile_\proto$, the exchange rate is always $x$ and the condition $\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}$ never holds,
\item in $\profile_\mathsf{ds}^\slot$, the exchange is always $0$ because the condition $\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}$ always holds.
\end{enumerate}
 This implies that there is $j^*\in[k-1]$ such that the condition  $\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}$ always holds in $\profile_{j^*+1}$ but with some probability $q>0$, the condition $\sum_{\party: \party\text{ double-signs in }\slot}\power_\party>\frac{1}{2}$ does not hold in $\profile_{j^*}$. Let $\party^*$ be the party that unilaterally deviates from $\profile_{j^*+1}$ to $\profile_{j^*}$.
\end{proof}
}


\subsubsection{Coordinated bribing attacks}\label{subsubsec:bribing_toy_coor}
We now study the scenario where the briber becomes more demanding, in the sense that it issues the parties' external rewards in a way that  the double-signing becomes effective (i.e., lead to the drop of the exchange rate). This implies some level of coordination among parties. Formally, for some fixed slot $\slot$, the external rewards are defined as
 \begin{equation}\label{eq:toy_external_coor}
\utilityBoost_{\party,\profile}(\trace)=\left\{\begin{array}{ll}\beta_\party,& \mbox{if in $\trace$, }\party\mbox{ double-signs in }\slot\\
0,&\mbox{otherwise}\end{array}\right.\;.
\end{equation}

In our study, we introduce the notion of an $\infractionPredicate_\mathsf{ds}$-agnostic strategy profile. 

\begin{definition}\label{def:ds_agnostic}
A strategy profile $\profile$ is \emph{$\infractionPredicate_\mathsf{ds}$-agnostic}, if for every $i,j\in[n]:i\neq j$, the strategy of $\party_i$ does not depend on the double-signing activity of $\party_j$ during the execution.
\end{definition}
Intuitively, the strategy of $\party_i$ in the $\infractionPredicate_\mathsf{ds}$-agnostic strategy profile $\profile$ does not contain clauses such as ``I will double-sign if $\party_j$ does not double-sign'', ``I will not double-sign, if everyone else has already double-signed'', etc.
%In the following theorem, we prove that in the coordinated setting, the strategy $\strategy_\mathsf{ds}^\slot$ strictly dominates every $\infractionPredicate_\mathsf{ds}$-agnostic strategy profile, if the party's bribe is sufficiently large.

\begin{theorem}\label{thm:toy_coor}
Let $\proto$ be a protocol with block-proportional rewards (cf. Subsection~\ref{subsec:preliminaries_proportion}) with $\reward$ rewards per block. Let $\profile_\proto$ denote the all-honest strategy profile. Assume that for any strategy profile $\sigma$, the exchange rate $\exchangeRate_\profile$ is defined as in Eq.~\eqref{eq:toy_exchange} and the external rewards $\utilityBoost_{\party,\profile}$ due to coordinated bribing \wrt slot $\slot$ are defined as in Eq.~\eqref{eq:toy_external_coor}. Let $\adversary$ be a synchronous router. Then, the following holds:

If $\beta_\party> E[\reward_{\party, \profile_\proto}]\cdot x$ for every party $\party\in\partySet$, then  $\profile_\mathsf{ds}^\slot$ is  $\epsilon$-reachable from $\profile_\proto$ \wrt Reward under $\adversary$, where $\epsilon$ is $\mathsf{negl}(\secparam)$.\TZ{Here, again complex strategies create problems and the proof breaks, unless we use an approximation factor. Need some time to think how the proof would go through}
\end{theorem}
\begin{proof}
We define the strategy profiles $\profile_j^\slot$, $j\in\{0,\ldots,n\}$  as in the proof of~\ref{thm:toy_nocoor_compliance}. in Theorem~\ref{thm:toy_nocoor}. Similarly, we can show that for every $j\in[n]$: (a) $\profile_j^\slot$ is unilateral deviation of $\party_j$ from $\profile_{j-1}^\slot$ and (b) $\utility_\party(\profile_j^\slot)> \utility_\party(\profile_{j-1}^\slot)$. By the definition of reachability, it suffices to show that for every $j\in[n]$, $\profile_j^\slot$ sets a best response for $\party_j$.

Let $\profile^*$ be a unilateral deviation of $\party_j$ from $\profile_{j-1}^\slot$. By definition of $\strategy_\mathsf{ds}^\slot$, $\profile_{j-1}^\slot$ is $\infractionPredicate_\mathsf{ds}$-agnostic, thus all the other parties' strategies in  $\profile^*$ (which are the same as in  $\profile_{j-1}^\slot$) do not depend on the double-signing activity of $\party_j$. Given the latter, we study the following cases:

\emph{Case 1}:  By unilaterally deviating from  $\profile_{j-1}^\slot$ to  $\profile_j^\slot$, the party $\party_j$'s double-signing  in slot $\slot$ does not affect the exchange rate. Then, the same holds for $\profile^*$. Let $D_\slot$ be the event that $\party_j$ double-signs in slot $\slot$ when following $\profile^*$. If the rate in $\profile_{j-1}^\slot$ and  $\profile_j^\slot$ is $c\in\{0,x\}$, we have that,
\begin{equation*}
\begin{split}
\utility_{\party_j}(\profile^*)&=\sum_z z\cdot\big(\Pr[D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot\exchangeRate_{\profile^*}+\utilityBoost_{\party_j, \profile^*}=z\mid D_\slot]+\\
&\quad+\Pr[\neg D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot\exchangeRate_{\profile^*}+\utilityBoost_{\party_j, \profile^*}=z\mid \neg D_\slot]\big)=\\
%
&\mbox{\TZ{Here, the proof breaks...:(}}\\
%
&=\sum_z z\cdot\big(\Pr[D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot c+\beta_{\party_j}=z]+\\
&\quad+\Pr[\neg D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot c=z]\big)=\\
%
&=\Pr[D_\slot]\cdot E[\reward_{\party_j, \profile^*}\cdot c+\beta_{\party_j}]+\Pr[\neg D_\slot]\cdot E[\reward_{\party_j, \profile^*}\cdot c]=\\
%
&= E[\reward_{\party_j, \profile^*}]\cdot c+\Pr[D_\slot]\cdot\beta_{\party_j}\leq E[\reward_{\party_j, \profile_\proto}]\cdot c+\beta_{\party_j}=\\
%
&=E[\reward_{\party_j, \profile_j^\slot}]\cdot c+\beta_{\party_j}=\utility_{\party_j}(\profile_j^\slot).
\end{split}
\end{equation*} 
%
\indent\emph{Case 2}:  By unilaterally deviating from  $\profile_{j-1}^\slot$ to  $\profile_j^\slot$, the party $\party_j$'s double-signing affects the exchange rate. In this case, by the definition of $\profile_1^\slot,\ldots,\profile_n^\slot$, it holds that 
%
\[\sum_{w=1}^{j-1}\power_{\party_w}\leq\frac{1}{2}\wedge\sum_{w=1}^{j}\power_{\party_w}>\frac{1}{2}.\]
%
Thus, if $D_\slot$ happens, then the exchange rate is $0$ and the external rewards of $\party_j$ are $\beta_{\party_j}$. If $D_\slot$ does not happen then the exchange rate is $x$ and, because we are in the coordinated setting, the external rewards of $\party_j$ are $0$. We have that
\begin{equation*}
\begin{split}
\utility_{\party_j}(\profile^*)&=\sum_z z\cdot\big(\Pr[D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot\exchangeRate_{\profile^*}+\utilityBoost_{\party_j, \profile^*}=z\mid D_\slot]+\\
&\quad+\Pr[\neg D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot\exchangeRate_{\profile^*}+\utilityBoost_{\party_j, \profile^*}=z\mid \neg D_\slot]\big)=\\
%
&=\sum_z z\cdot\big(\Pr[D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot 0+\beta_{\party_j}=z]+\\
&\quad+\Pr[\neg D_\slot]\cdot\Pr[\reward_{\party_j, \profile^*}\cdot x+0=z]\big)=\\
%
&=\Pr[D_\slot]\cdot \beta_{\party_j}+\Pr[\neg D_\slot]\cdot E[\reward_{\party_j, \profile^*}\cdot x]\leq\\
%
&\leq \mathsf{max}\{\beta_{\party_j}, E[\reward_{\party_j, \profile_\proto}]\cdot c\}=\beta_{\party_j}=\utility_{\party_j}(\profile_j^\slot).
\end{split}
\end{equation*} 
\end{proof}
